Segmentation-Free Outcome Prediction from Head and Neck Cancer PET/CT Images: Deep Learning-Based Feature Extraction from Multi-Angle Maximum Intensity Projections (MA-MIPs)

We introduce an innovative, simple, effective segmentation-free approach for outcome prediction in head \& neck cancer (HNC) patients. By harnessing deep learning-based feature extraction techniques and multi-angle maximum intensity projections (MA-MIPs) applied to Fluorodeoxyglucose Positron Emission Tomography (FDG-PET) volumes, our proposed method eliminates the need for manual segmentations of regions-of-interest (ROIs) such as primary tumors and involved lymph nodes. Instead, a state-of-the-art object detection model is trained to perform automatic cropping of the head and neck region on the PET volumes. A pre-trained deep convolutional neural network backbone is then utilized to extract deep features from MA-MIPs obtained from 72 multi-angel axial rotations of the cropped PET volumes. These deep features extracted from multiple projection views of the PET volumes are then aggregated and fused, and employed to perform recurrence-free survival analysis on a cohort of 489 HNC patients. The proposed approach outperforms the best performing method on the target dataset for the task of recurrence-free survival analysis. By circumventing the manual delineation of the malignancies on the FDG PET-CT images, our approach eliminates the dependency on subjective interpretations and highly enhances the reproducibility of the proposed survival analysis method.

==> Tables/E.tex <==

\begin{table}[H]
\footnotesize
% \tablesize
% \tiny
\medskip
% \setlength\tabcolsep{10pt}
    \centering
    \begin{tabular}{l|cccc|c|c} 
 % & \multicolumn{6}{c}{Fusion Methods}\\ \hline 
        % \hline
         Feature Extractor        & Mean                  & Median               & Max                    & STD-Dev               & ICA                   & AutoEncoder          \\ \hline
        \tiny{Global Average Pooling} &                   &                       &                       &                       &                       &                      \\ 
         EfficientNet Small (B1)  & $0.706\pm$\tiny{0.05} & $0.707\pm$\tiny{0.05} & $0.707\pm$\tiny{0.05} & $0.678\pm$\tiny{0.04} & $0.593\pm$\tiny{0.06} & $0.689\pm$\tiny{0.08}\\ 
         EfficientNet Medium (B4) & $0.615\pm$\tiny{0.03} & $0.638\pm$\tiny{0.03} & $0.626\pm$\tiny{0.05} & $0.640\pm$\tiny{0.04} & $0.590\pm$\tiny{0.08} & $0.644\pm$\tiny{0.05}\\ 
         EfficientNet Large  (B7) & $0.718\pm$\tiny{0.03} & $0.710\pm$\tiny{0.03} & $0.719\pm$\tiny{0.03} & $0.705\pm$\tiny{0.04} & $0.455\pm$\tiny{0.10} & $0.721\pm$\tiny{0.03}\\ 
                                  &                       &                       &                       &                       &                       &                      \\ 

        \tiny{Global Max Pooling} &                       &                       &                       &                       &                       &                      \\ 
         EfficientNet Small (B1)  & $0.613\pm$\tiny{0.08} & $0.613\pm$\tiny{0.07} & $0.703\pm$\tiny{0.06} & $0.680\pm$\tiny{0.03} & $0.541\pm$\tiny{0.03} & $0.639\pm$\tiny{0.06}\\ 
         EfficientNet Medium (B4) & $0.650\pm$\tiny{0.07} & $0.633\pm$\tiny{0.06} & $0.667\pm$\tiny{0.04} & $0.646\pm$\tiny{0.04} & $0.576\pm$\tiny{0.07} & $0.673\pm$\tiny{0.05}\\ 
         EfficientNet Large  (B7) & $0.625\pm$\tiny{0.03} & $0.634\pm$\tiny{0.03} & $0.697\pm$\tiny{0.05} & $0.665\pm$\tiny{0.04} & $0.459\pm$\tiny{0.03} & $0.651\pm$\tiny{0.03}\\
                                  &                       &                       &                       &                       &                       &                      \\ 
                                  
        \tiny{Global Median Pooling} &                    &                       &                       &                       &                       &                      \\ 
         EfficientNet Small (B1)  & $0.684\pm$\tiny{0.06} & $0.666\pm$\tiny{0.07} & $0.679\pm$\tiny{0.04} & $0.666\pm$\tiny{0.04} & $0.501\pm$\tiny{0.08} & $0.671\pm$\tiny{0.05}\\ 
         EfficientNet Medium (B4) & $0.652\pm$\tiny{0.02} & $0.663\pm$\tiny{0.03} & $0.651\pm$\tiny{0.04} & $0.641\pm$\tiny{0.05} & $0.491\pm$\tiny{0.03} & $0.630\pm$\tiny{0.06}\\ 
         EfficientNet Large  (B7) & $0.688\pm$\tiny{0.06} & $0.678\pm$\tiny{0.05} & $0.701\pm$\tiny{0.04} & $0.697\pm$\tiny{0.04} & $0.556\pm$\tiny{0.07} & $0.698\pm$\tiny{0.06}\\
                                  &                       &                       &                       &                       &                       &                      \\ 

        \tiny{Global STD-Dev Pooling} &                   &                       &                       &                       &                       &                      \\ 
         EfficientNet Small (B1)  & $0.702\pm$\tiny{0.05} & $0.701\pm$\tiny{0.06} & $0.701\pm$\tiny{0.06} & $0.709\pm$\tiny{0.02} & $0.456\pm$\tiny{0.05} & $0.685\pm$\tiny{0.08}\\ 
         EfficientNet Medium (B4) & $0.674\pm$\tiny{0.04} & $0.655\pm$\tiny{0.03} & $0.669\pm$\tiny{0.04} & $0.655\pm$\tiny{0.05} & $0.503\pm$\tiny{0.03} & $0.649\pm$\tiny{0.03}\\ 
         EfficientNet Large  (B7) & $0.708\pm$\tiny{0.04} & $0.706\pm$\tiny{0.04} & $0.713\pm$\tiny{0.04} & $0.689\pm$\tiny{0.06} & $0.506\pm$\tiny{0.04} & $0.665\pm$\tiny{0.04}\\ 
         
    \end{tabular}
    \caption{Caption}
    \label{tab:table_e}
\end{table}
